MRI-Free CT-to-Ultrasound Skull Registration in Transcranial Focused Ultrasound using CMUT based Integrated Therapeutic and Imaging Arrays

Accurate skull-to-array registration is essential for transcranial focused ultrasound (tFUS) because CT-derived skull models must be aligned with the physical-array coordinate system to support patient-specific aberration correction. Current workflows typically use MRI and/or external tracking to establish this spatial relationship, adding imaging infrastructure and coordinate transformations to the treatment workflow. Here, we describe an MRI-free CT-to-ultrasound registration framework using a hybrid hemispherical CMUT tFUS array that combines a sparse therapeutic array with an integrated CMUT US-Cross imaging array. The therapeutic array provides pulse-echo measurements of skull location, while the US-Cross array provides local high-resolution images of the skull surface. The approach was evaluated using a CT-derived outer cortical skull surface across a 25-pose matrix with 10-mm lateral offsets between the skull and array centers and +/-5 degree angular perturbations. Five randomized radial-noise seeds were applied to therapeutic pulse-echo measurements to model measurement or element-placement errors, yielding 125 pose-seed realizations per noise and active-element setting. US-Cross imaging features were generated using Field II and delay-multiply-and-sum plane-wave compounding. Four registration modes were evaluated: Therapeutic only, US-imaging only, Sequential, and Fused registration. Fused registration yielded the best overall performance, with a median total displacement error of 0.271 mm [0.169-0.420] and a median rotation error of 0.904 degrees [0.432-1.639]. These results support an all-ultrasound-based approach using a hybrid CMUT tFUS array for MRI-free CT-US skull registration.

==> latexmkrc <==
# Automatically compile standalone documents used by the xr package.
# Adapted from the Overleaf xr/latexmk example.

use File::Copy qw(copy);
use File::Basename qw(fileparse);

# Directory used for temporary output from supplementary compilation
$sub_doc_output = 'output-subdoc';

# Compile external documents using pdfLaTeX
@sub_doc_options = ('-pdf');

# Detect the missing .aux warning generated by xr
push @file_not_found, '^No file\\s*(.+)\\s*$';

# When a .tex -> .aux dependency is missing, compile the external document
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');

sub makeexternaldocument {
    if ($root_filename ne $_[0]) {

        my ($base_name, $path) = fileparse($_[0]);

        pushd $path;

        my $return = system(
            'latexmk',
            @sub_doc_options,
            "-aux-directory=$sub_doc_output",
            "-output-directory=$sub_doc_output",
            $base_name
        );

        if (($sub_doc_output ne '') && ($sub_doc_output ne '.')) {

            # Register the generated auxiliary file
            rdb_add_generated("$sub_doc_output/$base_name.aux");

            # Copy it beside supplement.tex so xr can find it
            copy(
                "$sub_doc_output/$base_name.aux",
                "$base_name.aux"
            );
        }

        popd;

        return $return;
    }
}

%$pdflatex = "latexdiff main.tex main2.tex > main-d.tex; pdflatex %O  main-d"

